Public Reaction to Scientific Research via Twitter Sentiment Prediction

Social media users share their ideas, thoughts, and emotions with other users. However, it is not clear how online users would respond to new research outcomes. This study aims to predict the nature of the emotions expressed by Twitter users toward scientific publications. Additionally, we investigate what features of the research articles help in such prediction. Identifying the sentiments of research articles on social media will help scientists gauge a new societal impact of their research articles.

==> ResearchObj.tex <==
\section{Research Objectives}

\hl{
The research objectives in this study can be divided into two major components:}
\begin{enumerate}[(1)]
\item To analyze trends of tweets for research articles for various research domains.
\item To understand the sentiment of tweets for research articles and build machine learning models to predict the sentiments of tweets.
\item To understand what research domains and what features of the paper play an important role in sentiment prediction of tweets.
\end{enumerate}

